Observation of Noise Suppression during High-Efficiency Wavelength Doubling of Intense Quasi-Monochromatic Laser Light

Ultra-stable, quasi-monochromatic laser light forms the basis for high-precision interferometric measurements, e.g. for observing gravitational waves and for time keeping with optical clocks. Optical frequency conversion enables access to wavelengths at which optical materials have the lowest absorption and the lowest mechanical loss. Here we report a 25 % reduction in relative intensity noise (of technical origin) when converting 1064 nm to 2128 nm for powers far above parametric oscillation threshold. The new wavelength has high potential for improving gravitational wave detection and other ultra-high-precision experiments as well. Our results provide a better understanding of the dynamics of nonlinear optical processes and have great potential for the stabilisation of laser sources in optical sensing and metrology.

==> packages.tex <==
%\usepackage{mathptmx}
\usepackage{xcolor}
\usepackage{siunitx}
\usepackage{graphicx}
\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{textcomp}
\usepackage{listings}
\usepackage{courier}
\usepackage{booktabs}
\usepackage{nicefrac, xfrac}

\lstset{
  basicstyle=\footnotesize\ttfamily,
  breaklines=true,
  xleftmargin=0.5cm}

\graphicspath{{img/}}

\hyphenation{Schna-bel}
%\newcommand{\todo}[1]{\textcolor[RGB]{214,39,40}%
    %{$\blacktriangleright$ #1 $\blacktriangleleft$}}
%\newcommand{\needsref}{\textcolor[RGB]{255,127,14}{[REF!]}}
\newcommand{\fixme}[1]{\textcolor[RGB]{255,127,14}{#1}}

\newcommand{\figref}[1]{figure~\ref{fig:#1}}
\newcommand{\gw}{gravitational wave}
\newcommand{\gws}{gravitational waves}
\newcommand{\gsw}{gravitational-wave}

\newcommand{\sqz}{\SI{7.2(2)}{dB}}
\newcommand{\asqz}{\SI{15.6(2)}{dB}}
\newcommand{\losses}{\SI{16.1(5)}{\%}}
\newcommand{\qe}{\SI{92(3)}{\%}}
\newcommand{\escapeEff}{\SI{98(1)}{\%}}
\newcommand{\efficiencyEstimated}{\SI{84(5)}{\%}}
\newcommand{\efficiencyMeasured}{\SI{83.9(5)}{\%}}
\newcommand{\pump}{\SI{1064}{nm}}
\newcommand{\convert}{\SI{2128}{nm}}

\def\eg{e.g.\ }
\sisetup{separate-uncertainty}


